Mutual Information Optimally Local Private Discrete Distribution Estimation

Consider statistical learning (e.g. discrete distribution estimation) with local $\epsilon$-differential privacy, which preserves each data provider's privacy locally, we aim to optimize statistical data utility under the privacy constraints. Specifically, we study maximizing mutual information between a provider's data and its private view, and give the exact mutual information bound along with an attainable mechanism: $k$-subset mechanism as results. The mutual information optimal mechanism randomly outputs a size $k$ subset of the original data domain with delicate probability assignment, where $k$ varies with the privacy level $\epsilon$ and the data domain size $d$. After analysing the limitations of existing local private mechanisms from mutual information perspective, we propose an efficient implementation of the $k$-subset mechanism for discrete distribution estimation, and show its optimality guarantees over existing approaches.

==> abandon.tex <==
When privacy level $\epsilon$ is in the low region (e.g. $\epsilon > \log(d)$), $1$-combination domain (e.g. the original data domain) is optimal,


The local differential privacy \cite{kasiviswanathan2011can}


The local differential privacy guarantees each data owner's privacy locally without trust on any other parties, such as the aggregator, the data curator, or other individuals.

Our bounds and the corresponding mechanism are applicable for any privacy levels, among which the intermediate regime $0.1\leq\epsilon\leq4.0$ is of great interests

The mechanism outperforms state-of-art approaches as demonstrated in theoretical and experimental results.

Local $\epsilon$-differential privacy guarantees each data owner's privacy locally and independently,

Intuitively, the local privacy controls ratio of likelihood of private views when secret value differs.


Note that the channel space $\mathcal{Z}$ is unlimited, and is not restricted to the original data domain $\mathcal{X}$, this has make the analyses of mutual information under local privacy much complicate than the noise channel cases.

&\leq \sum_{x \in \mathcal{X}} \frac{1}{d} max_{k'=1}^d\frac{(k'\cdot e^\epsilon \log{\frac{d\cdot e^\epsilon}{k'\cdot e^\epsilon+d-k'}}+(d-k')  \log{\frac{d}{k'\cdot e^\epsilon+d-k'}})}{(k'\cdot e^\epsilon +d-k')} &\\





We now deep into the additive structure of mutual information $I(x;\overline{z})$ in follows:
\begin{equation}\label{the:structure}
\begin{aligned}
&\ \ \ \ I(x;\overline{z})=\sum_{x \in \mathcal{X}} \sum_{k=0}^d {n \choose k} \frac{\overline{w}^{(d,k)}}{d}(k\cdot e^\epsilon \log{\frac{d\cdot e^\epsilon}{k\cdot e^\epsilon+d-k}}+(d-k)  \log{\frac{d}{k\cdot e^\epsilon+d-k}})&\\
&=\sum_{x \in \mathcal{X}} \sum_{k=0}^d {n \choose k} \frac{\overline{w}^{(d,k)} (k\cdot e^\epsilon +d-k)}{d}\frac{(k\cdot e^\epsilon \log{\frac{d\cdot e^\epsilon}{k\cdot e^\epsilon+d-k}}+(d-k)  \log{\frac{d}{k\cdot e^\epsilon+d-k}})}{(k\cdot e^\epsilon +d-k)}.&\\
\end{aligned}
\end{equation}

Note that $\sum_{k=0}^d {n \choose k} \overline{w}^{(d,k)} (k\cdot e^\epsilon +d-k)= 1.0$ as each row of $\overline{Q}$ is a valid probability distribution, we have following inequalities:
\begin{equation}\label{the:combination}
\begin{aligned}
&\ \ \ \ I(x;\overline{z})&\\
&\leq \sum_{x \in \mathcal{X}} \sum_{k=0}^d {n \choose k} \frac{\overline{w}^{(d,k)} (k\cdot e^\epsilon +d-k)}{d} max_{k'=0}^d\{\frac{k'\cdot e^\epsilon \log{\frac{d\cdot e^\epsilon}{k'\cdot e^\epsilon+d-k'}}+(d-k')  \log{\frac{d}{k'\cdot e^\epsilon+d-k'}}}{k'\cdot e^\epsilon +d-k'}\}&\\
&\leq max_{k=0}^d\{\frac{k\cdot e^\epsilon \log{\frac{d\cdot e^\epsilon}{k\cdot e^\epsilon+d-k}}+(d-k)  \log{\frac{d}{k\cdot e^\epsilon+d-k}}}{k\cdot e^\epsilon +d-k}\}.&\\
\end{aligned}
\end{equation}








We now deep into the additive structure of mutual information $I(x;\overline{z})$ in follows:
\begin{equation}\label{the:structure}
\begin{aligned}
&\ \ \ \ I(x;\overline{z})=\sum_{k=0}^d {n \choose k} \frac{\overline{w}^{(d,k)}}{d}(k\cdot e^\epsilon \log{\frac{d\cdot e^\epsilon}{k\cdot e^\epsilon+d-k}}+(d-k)  \log{\frac{d}{k\cdot e^\epsilon+d-k}})&\\
&=\sum_{k=0}^d {n \choose k} \frac{\overline{w}^{(d,k)} (k\cdot e^\epsilon +d-k)}{d}\frac{(k\cdot e^\epsilon \log{\frac{d\cdot e^\epsilon}{k\cdot e^\epsilon+d-k}}+(d-k)  \log{\frac{d}{k\cdot e^\epsilon+d-k}})}{(k\cdot e^\epsilon +d-k)}.&\\
\end{aligned}
\end{equation}

Note that $\sum_{k=0}^d {n \choose k} \frac{\overline{w}^{(d,k)} (k\cdot e^\epsilon +d-k)}{d}= 1.0$ as each row of $\overline{Q}$ is a valid probability distribution, we have following inequalities:
\begin{equation}\label{the:combination}
\begin{aligned}
&\ \ \ \ I(x;\overline{z})&\\
&\leq \sum_{k=0}^d {n \choose k} \frac{\overline{w}^{(d,k)} (k\cdot e^\epsilon +d-k)}{d} max_{k'=0}^d\{\frac{k'\cdot e^\epsilon \log{\frac{d\cdot e^\epsilon}{k'\cdot e^\epsilon+d-k'}}+(d-k')  \log{\frac{d}{k'\cdot e^\epsilon+d-k'}}}{k'\cdot e^\epsilon +d-k'}\}&\\
&\leq max_{k=0}^d\{\frac{k\cdot e^\epsilon \log{\frac{d\cdot e^\epsilon}{k\cdot e^\epsilon+d-k}}+(d-k)  \log{\frac{d}{k\cdot e^\epsilon+d-k}}}{k\cdot e^\epsilon +d-k}\}.&\\
\end{aligned}
\end{equation}




\begin{theorem}\label{the:bound} Let $X$ be a sample drawn according to the uniform distribution $P_u$ with $d$ states, and $Z$ be the locally $\epsilon$-differentially private view of $X$, the maximum mutual information between $X$ and $Z$ is as follows:
$$\sup_{Q\in M_\epsilon} I(X;Z) = .$$
\end{theorem}



\begin{theorem}\label{the:maxbound} Let $X$ be a sample drawn according to the uniform distribution $P_u$ with $d$ states, and $Z$ be the locally $\epsilon$-differentially private view of $X$, the maximum mutual information between $X$ and $Z$ is as follows:
$$\sup_{Q\in M_\epsilon} I(X;Z) = max_{k=0}^d\{\frac{k\cdot e^\epsilon \log{\frac{d\cdot e^\epsilon}{k\cdot e^\epsilon+d-k}}+(d-k)  \log{\frac{d}{k\cdot e^\epsilon+d-k}}}{k\cdot e^\epsilon +d-k}\}.$$
\end{theorem}


Now we interpret Theorem \ref{the:maxbound} and the corresponding optimal mechanism $Q^*$ in two special cases, including $e^\epsilon \ll d$ and $e^\epsilon \gg d$, and build connection with existing mechanisms for private discrete distribution estimation.

Note that the channel space $\mathcal{Z}$ is unlimited, and is not restricted to the original data domain $\mathcal{X}$, this has made the analyses of mutual information under local private constraints much challenging than the traditional noise channel cases.


Denote $k^*$ as the corresponding $k$ that maximizes $I_k={\frac{k\cdot e^\epsilon \log{\frac{d\cdot e^\epsilon}{k\cdot e^\epsilon+d-k}}+(d-k)  \log{\frac{d}{k\cdot e^\epsilon+d-k}}}{k\cdot e^\epsilon +d-k}}$, the bound in Corollary (\ref{the:max}) is achievable when ${n \choose k^*} \overline{w}^{(d,k^*)}=\frac{d}{k^*\cdot e^\epsilon +d-k^*}$ and $\overline{w}^{(d,k)}=0.0$ for $k\neq k^*$, we denote this kind ofmechanism as $Q^*$. Indeed, since $I_{k}$ is concave when real value ${k}$ ranges from $0$ to $d$, the $\beta=\frac{(\epsilon e^\epsilon -e^\epsilon+1) d}{(e^\epsilon-1)^2}$ maximize $I_{\beta}$, hence $k^*=\lfloor\beta\rfloor$ or $k^*=\lceil\beta\rceil$  (see detail in Appendix ??).



In concise, there is an at-least $e^{-0.5 \epsilon}$ multiplicative gap in mutual information perspective between $Q^b$ and an mutual information optimal mechanism $Q^{k^*}$. Practically, when $\epsilon$ is relatively small (e.g. $\epsilon < 0.2$), the gap is bounded by a small factor, but when $\epsilon$ getting larger, the gap becomes unacceptable at exponential speed.


But such an estimator suffers from $\Theta({d \choose k})$ memory costs and $\Omega()$


Consider $n$ data providers, each provider holds a secret value $x_i \in \mathcal{X}$, where $\mathcal{X}=\{X_j\}_{i=1}^d$ is the data domain of size $d$. The truly discrete distribution $\theta$ over population can be expressed as $\theta_j = \frac{1}{n}\#\{j: x_i=X_j\}$. In the local setting of differential privacy, each data provider locally and dependently sanitizes $x_i$ through a local $\epsilon$-differential private channel $Q_i$, and obtains a private view $z_i \in \mathcal{Z}$ of $x_i$, where $\mathcal{Z}=\{Z_l\}_{l=1}^{|\mathcal{Z}|}$ is the output alphabets or channel space. The $z_i$ instead of $x_i$ is published to untrusted data aggregator, who infers a estimation of the truly distribution $\theta$ from observed private views $\{z_i\}_{i=1}^n$.


In concise, existing private mechanisms for discrete distribution estimation performs poorly for intermediate privacy region from mutual information perspective. Fortunately, the process in proving the mutual information bound under local $\epsilon$-differential privacy naturally induces a mutual information optimal mechanism, the $k$-subset mechanism. In following section, we focus on practical implementing of $k$-subset mechanism, for discrete distribution estimation and its performance under more specific distribution estimation performance metrics, such as $l_2$-error and $l_1$-error, instead of mutual information metric in here.


As defined in Definition \ref{def:kcombination}, $k$-subset mechanism randomly response with a size $k$ subset $Z$ of the original private data domain $\mathcal{X}$.

\begin{equation*}
E[f(X_j)]=n\cdot\theta_j\cdot \frac{k e^\epsilon}{k e^\epsilon +d-k}+n\cdot(1-\theta_j)\cdot(\frac{k e^\epsilon}{k e^\epsilon +d-k}\cdot \frac{k-1}{d-1}+\frac{d-k}{k e^\epsilon +d-k}\cdot \frac{k}{d-1}).
\end{equation*}

we have $I''(\beta)=-\frac{e^{-2\epsilon}(e^\epsilon-1)^4}{d^2 \epsilon^2}\leq 0$



Note that almost all existing private mechanisms for distribution estimation are special cases of $Q$ in Theorem \ref{the:l2koptimal}, including binary randomized response \citep{duchi2013localnips}\citep{duchi2013local}\citep{erlingsson2014rappor}, multivariate randomized response \citep{warner1965randomized}\citep{mcsherry2007mechanism}\citep{kairouz2014extremal}, $1$-bit protocol \citep{bassily2015local}\citep{chen2016private}. Hence, $k$-subset mechanism outperforms these state-of-art mechanisms.



We notice that there are some other local private mechanisms by adding noise (e.g. Laplace noise \citep{dwork2006calibrating}, two-sided geometric noises \citep{ghosh2009universally}) on secret data that represented as bit maps, but their estimation accuracies or statistical utilities are rigidly dominated by the binary randomized response mechanism. Consequently, only the binary randomized response mechanism and multivariate randomized response mechanism are necessarily analysed here.

\subsubsection{Discussion}
As the analyse results show, binary randomized response mechanism $Q^b$ is suitable when $\epsilon$ is relatively small (e.g. $\epsilon < 0.2$), and multivariate randomized response mechanism $Q^m$ is suitable when $\epsilon$ is relatively large (e.g. $\frac{(e^\epsilon-1)^2}{\epsilon e^\epsilon - e^\epsilon+1} \geq \frac{d}{2}$). What's worse, both $Q^b$ and $Q^m$ fails in the intermediate privacy region.


Numerical results are the logarithm of mean error of $80$ repeated simulations.


\cline{2-12}
& $5.0$ &  0.000292	& 4.60e-05	& 4.57e-05	& \textbf{4.52e-05} 	&  0.07727	& 0.03039	& 0.03025	& \textbf{0.03004} 	& 1 	& 1 \\

$0.01$ &  0.6776	& 0.8968	& 0.6968	& 0.6831 	&  1.934	& 1.96	& 1.935	& 1.933 	& 32 	& 32\\
\cline{2-12}
&

& $0.5$ &  0.03503	& 0.1355	& 0.03454	& 0.03423 	&  1.431	& 1.812	& 1.428	& 1.422 	& 53 	& 48 \\




\begin{table}[H]\label{tab:results}
\setlength\tabcolsep{0.85ex}
\renewcommand{\arraystretch}{1.20}
\caption{Mean $\|\hat{\theta}-\theta\|_2^2$ and $\|\hat{\theta}-\theta\|_1$ error results for discrete distribution estimation.}
\small
\centering
\renewcommand{\multirowsetup}{\centering}
\begin{tabular}{|c|c|c|c|c|c||c|c|c|c|c|c|}
\cline{3-10}

\multicolumn{2}{c}{}  & \multicolumn{4}{|c||}{\large{$\mathbf{\|\hat{\theta}-\theta\|_2^2}$}} & \multicolumn{4}{c}{\large{$\mathbf{\|\hat{\theta}-\theta\|_1}$}} & \multicolumn{2}{|c}{} \\
\cline{1-12}

$d=$& $\epsilon=$  & \textbf{BRR} & \textbf{MRR} & $\mathbf{k^*}$\textbf{-SS} & $\mathbf{k^\#}$\textbf{-SS}& \textbf{BRR} & \textbf{MRR} & $\mathbf{k^*}$\textbf{-SS} & $\mathbf{k^\#}$\textbf{-SS} & $\mathbf{k^*}$ & $\mathbf{k^\#}$ \\
\hline

\multicolumn{1}{|c|}{\multirow{2}{*}{2}} & $0.1$ &  0.03361	& 0.009983	& 0.01001	& \textbf{0.009026} 	&  0.2058	& 0.1123	& 0.1132	& \textbf{0.1048} 	& 1 	& 1 \\
\cline{2-12}
& $1.0$ &  0.00043	& 9.75e-05	& 9.82e-05	& \textbf{8.21e-05} 	&  0.02341	& 0.01112	& 0.01084	& \textbf{0.01024} 	& 1 	& 1 \\
\cline{1-12}

\multicolumn{1}{|c|}{\multirow{4}{*}{4}} & $0.01$ &  0.6492	& 0.604	& \textbf{0.5797}	& 0.5822 	&  1.313	& 1.271	& \textbf{1.233}	& 1.242 	& 2 	& 2 \\
\cline{2-12}
& $0.1$ &  0.09319	& 0.06928	& 0.05542	& \textbf{0.05383} 	&  0.4863	& 0.4194	& 0.3728	& \textbf{0.3683} 	& 2 	& 2 \\
\cline{2-12}
& $0.5$ &  0.004279	& 0.00286	& \textbf{0.002628}	& 0.002767 	&  0.1044	& 0.08596	& \textbf{0.08118}	& 0.08458 	& 2 	& 2 \\
\cline{2-12}
& $1.0$ &  0.001135	& \textbf{0.000526}	& 0.000566	& 0.000564 	&  0.05362	& \textbf{0.03664}	& 0.03828	& 0.03787 	& 1 	& 1 \\
\cline{1-12}


\multicolumn{1}{|c|}{\multirow{4}{*}{6}} & $0.01$ &  0.6523	& 0.6956	& 0.6366	& \textbf{0.6356} 	&  1.47	& 1.51	& \textbf{1.45}	& \textbf{1.45} 	& 3 	& 3 \\
\cline{2-12}
& $0.1$ &  0.1195	& 0.1333	& \textbf{0.09006}	& 0.09741 	&  0.6773	& 0.7154	& \textbf{0.5851}	& 0.6112 	& 3 	& 3 \\
\cline{2-12}
& $0.5$ &  0.007409	& 0.006899	& 0.005201	& \textbf{0.00512} 	&  0.1664	& 0.162	& 0.14	& \textbf{0.1398} 	& 3 	& 2 \\
\cline{2-12}
& $1.0$ &  0.001851	& 0.00138	& 0.001216	& \textbf{0.001192} 	&  0.08388	& 0.0723	& 0.06813	& \textbf{0.06764} 	& 2 	& 2 \\
\cline{1-12}


\multicolumn{1}{|c|}{\multirow{5}{*}{8}} & $0.01$ &  0.7177	& 0.7516	& \textbf{0.6477}	& 0.6769 	&  1.613	& 1.633	& \textbf{1.558}	& 1.586 	& 4 	& 4 \\
\cline{2-12}
& $0.1$ &  0.1367	& 0.184	& 0.1186	& \textbf{0.1176} 	&  0.831	& 0.9464	& 0.7708	& \textbf{0.7654} 	& 4 	& 4 \\
\cline{2-12}
& $0.5$ &  0.01015	& 0.01189	& 0.007975	& \textbf{0.007868} 	&  0.2272	& 0.2457	& 0.2003	& \textbf{0.1994} 	& 3 	& 3 \\
\cline{2-12}
& $1.0$ &  0.002501	& 0.002405	& 0.001958	& \textbf{0.001902} 	&  0.1124	& 0.1103	& 0.09971	& \textbf{0.09808} 	& 3 	& 2 \\
\cline{2-12}
&$2.0$ 	&  0.000621	& 0.000314	& 0.000405	& \textbf{0.000313} 	&  0.05651	& 0.04001	& 0.04565	& \textbf{0.03976} 	& 2 	& 1 \\
\cline{1-12}

\multicolumn{1}{|c|}{\multirow{6}{*}{16}} & $0.01$ &  0.7008	& 0.8152	& \textbf{0.6988}	& 0.7109 	&  1.77	& 1.819	& \textbf{1.767}	& 1.777 	& 8 	& 8 \\
\cline{2-12}
& $0.1$ &  0.1593	& 0.2754	& 0.1535	& \textbf{0.1511} 	&  1.188	& 1.431	& 1.178	& \textbf{1.166} 	& 8 	& 8 \\
\cline{2-12}
& $0.5$ &  0.01976	& 0.03955	& 0.017	& \textbf{0.01677} 	&  0.4442	& 0.6302	& 0.4127	& \textbf{0.4097} 	& 7 	& 6 \\
\cline{2-12}
& $1.0$ &  0.005306	& 0.008367	& 0.004468	& \textbf{0.004349} 	&  0.2304	& 0.2896	& 0.2117	& \textbf{0.2086} 	& 5 	& 4 \\
\cline{2-12}
&$2.0$ 	&  0.001315	& 0.000938	& 0.000907	& \textbf{0.000851} 	&  0.1157	& 0.09716	& 0.09577	& \textbf{0.09265} 	& 3 	& 2 \\
\cline{2-12}
&$3.0$ 	&  0.000548	& \textbf{0.000207}	& 0.000295	& 0.000209 	&  0.07454	& \textbf{0.04555}	& 0.05492	& 0.04567 	& 2 	& 1 \\
\cline{1-12}

\multicolumn{1}{|c|}{\multirow{7}{*}{32}} & $0.01$ &  0.7025	& 0.8804	& \textbf{0.6925}	& 0.6969 	&  1.878	& 1.919	& 1.879	& \textbf{1.875} 	& 16 	& 16\\
\cline{2-12}
& $0.1$ &  0.161	& 0.3684	& \textbf{0.1555}	& 0.1565 	&  1.484	& 1.739	& \textbf{1.469}	& 1.487 	& 15 	& 15 \\
\cline{2-12}
& $0.5$ &  0.02918	& 0.07496	& \textbf{0.02794}	& 0.02807 	&  0.7602	& 1.158	& 0.7457	& \textbf{0.7451} 	& 13 	& 12 \\
\cline{2-12}
& $1.0$ &  0.009706	& 0.02396	& 0.008989	& \textbf{0.008763} 	&  0.4393	& 0.6923	& 0.4256	& \textbf{0.418} 	& 11 	& 9 \\
\cline{2-12}
& $1.5$ &  0.004731	& 0.00822	& 0.004004	& \textbf{0.003848} 	&  0.3074	& 0.4042	& 0.2838	& \textbf{0.2779} 	& 9 	& 6 \\
\cline{2-12}
&$2.0$ 	&  0.002608	& 0.003078	& 0.002108	& \textbf{0.001878} 	&  0.2285	& 0.2476	& 0.2059	& \textbf{0.1954} 	& 7 	& 4 \\
\cline{2-12}
&$3.0$ 	&  0.001102	& 0.000555	& 0.000736	& \textbf{0.000549} 	&  0.1495	& 0.1053	& 0.1221	& \textbf{0.1051} 	& 4 	& 2 \\
\cline{1-12}

\multicolumn{1}{|c|}{\multirow{7}{*}{64}} & $0.1$ &  0.1543	& 0.4348	& 0.1536	& \textbf{0.1519} 	&  1.691	& 1.88	& \textbf{1.69}	& \textbf{1.69} 	& 31 	& 30 \\
\cline{2-12}
& $0.5$ &  0.03388	& 0.105	& \textbf{0.03359}	& 0.03383 	&  1.114	& 1.578	& \textbf{1.107}	& 1.11 	& 27 	& 24 \\
\cline{2-12}
& $1.0$ &  0.01476	& 0.04257	& 0.01414	& \textbf{0.01383} 	&  0.7649	& 1.213	& 0.7439	& \textbf{0.7397} 	& 22 	& 17 \\
\cline{2-12}
& $1.5$ &  0.007885	& 0.01927	& 0.007198	& \textbf{0.006802} 	&  0.5603	& 0.8649	& 0.5343	& \textbf{0.5209} 	& 17 	& 12 \\
\cline{2-12}
&$2.0$ 	&  0.004758	& 0.008823	& 0.004027	& \textbf{0.00368} 	&  0.4358	& 0.5903	& 0.3998	& \textbf{0.3823} 	& 13 	& 8 \\
\cline{2-12}
&$3.0$ 	&  0.002059	& 0.001614	& 0.001413	& \textbf{0.001128} 	&  0.2872	& 0.2538	& 0.2382	& \textbf{0.212} 	& 7 	& 3 \\
\cline{2-12}
&$5.0$ 	&  0.000576	& 9.97e-05	& 0.000189	& \textbf{9.95e-05} 	&  0.1523	& 0.06337	& 0.0873	& \textbf{0.06334} 	& 2 	& 1 \\
\cline{1-12}

\multicolumn{1}{|c|}{\multirow{5}{*}{$2^7$}} & $0.1$ &  0.148	& 0.523	& \textbf{0.1431}	& 0.1456 	&  1.824	& 1.95	& \textbf{1.823}	& 1.824 	& 62 	& 61 \\
\cline{2-12}
& $1.0$ &  0.01723	& 0.05896	& 0.01675	& \textbf{0.01658} 	&  1.122	& 1.61	& 1.108	& \textbf{1.103} 	& 43 	& 34 \\
\cline{2-12}
&$2.0$ 	&  0.00715	& 0.01694	& 0.006344	& \textbf{0.00591} 	&  0.7504	& 1.107	& 0.7083	& \textbf{0.6832} 	& 26 	& 15 \\
\cline{2-12}
&$3.0$ 	&  0.003583	& 0.004364	& 0.002627	& \textbf{0.002223} 	&  0.5339	& 0.5858	& 0.4573	& \textbf{0.4203} 	& 14 	& 6 \\
\cline{2-12}
&$5.0$ 	&  0.001098	& 0.000240	& 0.000465	& \textbf{0.000239} 	&  0.2964	& \textbf{0.1379}	& 0.1934	& 0.1385 	& 4 	& 1 \\
\cline{1-12}

\multicolumn{1}{|c|}{\multirow{4}{*}{$2^8$}} & $1.0$ &   0.01753	& 0.07743	& 0.01726	& \textbf{0.01703} 	&  1.432	& 1.83	& 1.424	& \textbf{1.417} 	& 87 	& 69 \\
\cline{2-12}
&$2.0$ 	&  0.008458	& 0.02386	& 0.007801	& \textbf{0.007354} 	&  1.112	& 1.539	& 1.077	& \textbf{1.049} 	& 53 	& 31 \\
\cline{2-12}
&$3.0$ 	&  0.004899	& 0.008265	& 0.003999	& \textbf{0.003455} 	&  0.8757	& 1.093	& 0.7928	& \textbf{0.7389} 	& 29 	& 12 \\
\cline{2-12}
&$5.0$ 	&  0.001868	& 0.0005986	& 0.0008629	& \textbf{0.000546} 	&  0.5447	& 0.3074	& 0.3707	& \textbf{0.2944} 	& 7 	& 2 \\
\cline{1-12}


\hline
\end{tabular}
\end{table}


Specifically, the binary randomized response achieves optimal estimation accuracy up to a constant in the high privacy region, while multivariate randomized response mechanism achieves optimal asymptotic accuracy when $\epsilon$ approaches $+\infty$. However, as we will show in following, there are significant mutual information gaps for both of these two mechanisms in the intermediate privacy region (e.g. $\leq \epsilon \leq $), which is practically commonly deployed privacy region.

Deep into the conditional probabilities of $Q^m$ and the $k$-subset mechanism in Definition \ref{def:kcombination}, we observe that $Q^{m}$ is actually equivalent to $1$-subset mechanism $Q^{1}$ where only the columns with one $e^\epsilon$ in pattern matrix have non-zero weights, its mutual information is $I_1$.

The mutual information $I(Z;X)$ between private view $Z$ under $Q^m$ and the no-prior-knowledge secret data $X$ is ${\frac{e^\epsilon \log{\frac{d\cdot e^\epsilon}{e^\epsilon+d-k}}+(d-1)  \log{\frac{d}{e^\epsilon+d-1}}}{e^\epsilon +d-1}}$, which is also the upper bound of mutual information or channel capacity under $Q^m$.

In previous section, existing private mechanisms for discrete distribution estimation are analysed to be performing poorly for intermediate privacy region from mutual information perspective. Fortunately, the process in proving the mutual information bound under local $\epsilon$-differential privacy naturally induces a mutual information optimal mechanism, the $k$-subset mechanism.

Note that the channel space $\mathcal{Z}$ is unlimited,
and is not restricted to the original data domain $\mathcal{X}$,
this has made the analyses of mutual information under local private constraints much challenging than the traditional noise channel cases.

where $I_{k^*}$ is the maximal $I_k$ when $k\in[0,d]$, $I_{k^*}$ is also the mutual information upper bound under private constraints as discussed around Corollary \ref{the:max}.

In concise, the $Q^m$ is a mutual information optimal mechanism only when $I_1\geq I_2$, or roughly when $\beta=\frac{(\epsilon e^\epsilon - e^\epsilon+1) d}{(e^\epsilon-1)^2}$ in Theorem \ref{the:maxbound} is smaller than about $2$, while when $\frac{(e^\epsilon-1)^2}{\epsilon e^\epsilon - e^\epsilon+1} \leq \frac{d}{2}$, the mechanism $Q^m$ is unable to fully capture mutual information under local $\epsilon$-differential private constraints.

Actually $Q^{m}$ is  equivalent to $1$-subset mechanism $Q^{1}$ where only the columns with one $e^\epsilon$ in pattern matrix have non-zero weights, its mutual information is $I_1$.

The mutual information $I(Z;X)$ between private view $Z$ under $Q^m$ and the no-prior-knowledge secret data $X$ is ${\frac{e^\epsilon \log{\frac{d\cdot e^\epsilon}{e^\epsilon+d-k}}+(d-1)  \log{\frac{d}{e^\epsilon+d-1}}}{e^\epsilon +d-1}}$. Actually $Q^{m}$ is  equivalent to $1$-subset mechanism $Q^{1}$ where only the columns with one $e^\epsilon$ in pattern matrix have non-zero weights, its mutual information is $I_1$.


Working under local $\epsilon$-differential privacy constraints which rigourously preserve differential privacy locally over a data domain, we study the problem of maximizing mutual information between no-prior-knowledge secret data and observed private data, and its application to discrete distribution estimation. We firstly give exact bounds on the mutual information and provide a concrete attainable mechanism. The mutual-information-optimal mechanism implies that resorting to power set of the original data domain as output alphabet for local differential privacy preserving is not more favorable than a certain $k$-combination domain. We then build close connection between the mutual-information-optimal mechanism and state-of-art local private discrete distribution mechanisms that are based on binary randomized response or multi-variate randomized response, and show their statistical inefficiencies under commonly used intermediate-region privacy levels (e.g. $\epsilon\geq 0.2$ and $\frac{(e^\epsilon-1)^2}{\epsilon e^\epsilon - e^\epsilon+1} \leq \frac{d}{2}$). Both theoretical and experimental results demonstrate significant advantages of the $k$-combination mechanism for distribution estimation over randomized response based techniques since $1965$.

To prove Theorem \ref{the:maxbound} and give the concrete mechanism reach the bound, we firstly introduce combinatorial representation of optimal mechanisms under local privacy established by \citet{kairouz2014extremal}.

Follow \citep{kairouz2014extremal}, we call mechanisms that satisfying such properties as staircase mechanisms.


\textbf{Future work.}\,\,\,
An important research direction is the universal mutual information bound ( or channel capacity ) under local privacy, which includes analysing whether the mutual information bound in Theorem \ref{the:maxbound} holds in interactive setting or for $X$ with prior knowledge, and seeking for the optimal domain size $d$ that maximizes mutual information bound. Similar to Corollary \ref{the:max} and Theorem \ref{the:l2koptimal}, another research direction is theoretically characterizing performance of $k$-subset mechanism under other measurements (e.g. $l_1$-norm, $l_\infty$-norm).
\vspace*{-1em}


Similar to Corollary \ref{the:max} and Theorem \ref{the:l2koptimal}, another research direction is theoretically characterizing performance of $k$-subset mechanism under other measurements (e.g. $l_1$-norm, $l_\infty$-norm).

& $0.5$ &  0.02918	& 0.07496	& \textbf{0.02794}	& 0.02807 	&  0.7602	& 1.158	& 0.7457	& \textbf{0.7451} 	& 13 	& 12 \\
\cline{2-12}



@inproceedings{wang2016private,
  title={Private Weighted Histogram Aggregation in Crowdsourcing},
  author={Wang, Shaowei and Huang, Liusheng and Wang, Pengzhan and Deng, Hou and Xu, Hongli and Yang, Wei},
  booktitle={Wireless Algorithms, Systems, and Applications},
  year={2016},
  publisher={Springer}
}

@incollection{hsu2012distributed,
  title={Distributed private heavy hitters},
  author={Hsu, Justin and Khanna, Sanjeev and Roth, Aaron},
  booktitle={ICALP},
  year={2012},
  publisher={Springer}
}

Specifically, for the fundamental task of private learning: discrete distribution estimation, convergence rate bounds along with attainable mechanisms in the high privacy regime where $\epsilon < 1$ have been well studied (e.g. in \citep{duchi2013local}\citep{bassily2015local}). However, in the more practical region of privacy levels, such as $0.1\leq\epsilon\leq4$, in view of statistical utility, there is still much potential can be squeezed under local differential privacy constraints.


In this work, from statistical utility perspective, we study discrete distribution estimation with maximized mutual information under the local $\epsilon$-differential privacy setting. More specifically, we focus on non-adaptive statistical inference without prior knowledge is available for each owner with secret data. Our work benefits from the corner property of optimal mechanism maximizing mutual information under local privacy in work \citep{kairouz2014extremal}, and gives a much stronger result shows that exponential sized patterns of ratio on output likelihood is unnecessary but a certain $k$-combination patterns is optimality achievable. Motivated by this result and its corresponding optimal mechanism, similar results for local private discrete distribution estimation with both $L_1$ and $L_2$ error measurements are formally analysed.

We give exact mutual information bounds under local privacy, and observe statistical utility gap of existing mechanisms for private discrete distribution estimation. Suggested by the concrete mechanism achieving maximal mutual information, we then present the $k$-combination mechanism, and analyse its significant theoretical advantages over existing estimation mechanisms, especially in the intermediate privacy regime where $\epsilon\geq 0.2$ and $\frac{(e^\epsilon-1)^2}{\epsilon e^\epsilon - e^\epsilon+1} \leq \frac{d}{2}$, both $L_1$ (total variation) and $L_2$ error of estimated distribution are analysed. We also deduce an equivalent estimator for the $k$-combination mechanism in a simple form, which makes the mechanism highly efficient. In concise, guided by mutual information maximization process, a statistical and computational efficient local privacy discrete distribution estimation mechanism, the $k$-combination mechanism, is introduced in this work.






\begin{table}[H]
\setlength\tabcolsep{0.81ex}
\renewcommand{\arraystretch}{1.12}
\caption{Simulation results of mean $\|\hat{\theta}-\theta\|_2^2$ and $\|\hat{\theta}-\theta\|_1$ error for discrete distribution estimation.}
\small
\centering
\renewcommand{\multirowsetup}{\centering}
\label{tab:result}
\begin{tabular}{|c|c||c|c|c|c||c|c|c|c||c|c|}
\cline{3-10}

\multicolumn{2}{c}{}  & \multicolumn{4}{|c||}{\large{$\mathbf{\|\hat{\theta}-\theta\|_2^2}$}} & \multicolumn{4}{c}{\large{$\mathbf{\|\hat{\theta}-\theta\|_1}$}} & \multicolumn{2}{|c}{} \\
\cline{1-12}

$d=$& $\epsilon=$  & \textbf{BRR} & \textbf{MRR} & $\mathbf{k^*}$\textbf{-SS} & $\mathbf{k^\#}$\textbf{-SS}& \textbf{BRR} & \textbf{MRR} & $\mathbf{k^*}$\textbf{-SS} & $\mathbf{k^\#}$\textbf{-SS} & $\mathbf{k^*}$ & $\mathbf{k^\#}$ \\
\hline

\multicolumn{1}{|c|}{\multirow{2}{*}{2}} & $0.1$ &  0.03361	& 0.009983	& 0.01001	& \textbf{0.009026} 	&  0.2058	& 0.1123	& 0.1132	& \textbf{0.1048} 	& 1 	& 1 \\
\cline{2-12}
& $1.0$ &  0.00043	& 9.75e-05	& 9.82e-05	& \textbf{8.21e-05} 	&  0.02341	& 0.01112	& 0.01084	& \textbf{0.01024} 	& 1 	& 1 \\
\cline{1-12}

\multicolumn{1}{|c|}{\multirow{4}{*}{4}} & $0.01$ &  0.6492	& 0.604	& \textbf{0.5797}	& 0.5822 	&  1.313	& 1.271	& \textbf{1.233}	& 1.242 	& 2 	& 2 \\
\cline{2-12}
& $0.1$ &  0.09319	& 0.06928	& 0.05542	& \textbf{0.05383} 	&  0.4863	& 0.4194	& 0.3728	& \textbf{0.3683} 	& 2 	& 2 \\
\cline{2-12}
& $0.5$ &  0.00427	& 0.00286	& \textbf{0.00262}	& 0.00276 	&  0.1044	& 0.08596	& \textbf{0.08118}	& 0.08458 	& 2 	& 2 \\
\cline{2-12}
& $1.0$ &  0.0011	& \textbf{0.00052}	& 0.00056	& 0.00056 	&  0.05362	& \textbf{0.03664}	& 0.03828	& 0.03787 	& 1 	& 1 \\
\cline{1-12}


\multicolumn{1}{|c|}{\multirow{4}{*}{6}} & $0.01$ &  0.6523	& 0.6956	& 0.6366	& \textbf{0.6356} 	&  1.47	& 1.51	& \textbf{1.45}	& \textbf{1.45} 	& 3 	& 3 \\
\cline{2-12}
& $0.1$ &  0.1195	& 0.1333	& \textbf{0.09006}	& 0.09741 	&  0.6773	& 0.7154	& \textbf{0.5851}	& 0.6112 	& 3 	& 3 \\
\cline{2-12}
& $0.5$ &  0.00740	& 0.00689	& 0.00520	& \textbf{0.00512} 	&  0.1664	& 0.162	& 0.14	& \textbf{0.1398} 	& 3 	& 2 \\
\cline{2-12}
& $1.0$ &  0.00185	& 0.00138	& 0.001216	& \textbf{0.00119} 	&  0.08388	& 0.0723	& 0.06813	& \textbf{0.06764} 	& 2 	& 2 \\
\cline{1-12}


\multicolumn{1}{|c|}{\multirow{5}{*}{8}} & $0.01$ &  0.7177	& 0.7516	& \textbf{0.6477}	& 0.6769 	&  1.613	& 1.633	& \textbf{1.558}	& 1.586 	& 4 	& 4 \\
\cline{2-12}
& $0.1$ &  0.1367	& 0.184	& 0.1186	& \textbf{0.1176} 	&  0.831	& 0.9464	& 0.7708	& \textbf{0.7654} 	& 4 	& 4 \\
\cline{2-12}
& $0.5$ &  0.01015	& 0.01189	& 0.00797	& \textbf{0.00786} 	&  0.2272	& 0.2457	& 0.2003	& \textbf{0.1994} 	& 3 	& 3 \\
\cline{2-12}
& $1.0$ &  0.0025	& 0.00241	& 0.00195	& \textbf{0.00190} 	&  0.1124	& 0.1103	& 0.09971	& \textbf{0.09808} 	& 3 	& 2 \\
\cline{2-12}
&$2.0$ 	&  0.00062	& 0.00032	& 0.0004	& \textbf{0.00031} 	&  0.05651	& 0.04001	& 0.04565	& \textbf{0.03976} 	& 2 	& 1 \\
\cline{1-12}

\multicolumn{1}{|c|}{\multirow{6}{*}{16}} & $0.01$ &  0.7008	& 0.8152	& \textbf{0.6988}	& 0.7109 	&  1.77	& 1.819	& \textbf{1.767}	& 1.777 	& 8 	& 8 \\
\cline{2-12}
& $0.1$ &  0.1593	& 0.2754	& 0.1535	& \textbf{0.1511} 	&  1.188	& 1.431	& 1.178	& \textbf{1.166} 	& 8 	& 8 \\
\cline{2-12}
& $0.5$ &  0.01976	& 0.03955	& 0.017	& \textbf{0.01677} 	&  0.4442	& 0.6302	& 0.4127	& \textbf{0.4097} 	& 7 	& 6 \\
\cline{2-12}
& $1.0$ &  0.00531	& 0.00837	& 0.00447	& \textbf{0.00434} 	&  0.2304	& 0.2896	& 0.2117	& \textbf{0.2086} 	& 5 	& 4 \\
\cline{2-12}
&$2.0$ 	&  0.00132	& 0.00094	& 0.00091	& \textbf{0.00085} 	&  0.1157	& 0.09716	& 0.09577	& \textbf{0.09265} 	& 3 	& 2 \\
\cline{2-12}
&$3.0$ 	&  0.00055	& \textbf{0.0002}	& 0.000295	& 0.00021 	&  0.07454	& \textbf{0.04555}	& 0.05492	& 0.04567 	& 2 	& 1 \\
\cline{1-12}

\multicolumn{1}{|c|}{\multirow{6}{*}{32}} & $0.01$ &  0.7025	& 0.8804	& \textbf{0.6925}	& 0.6969 	&  1.878	& 1.919	& 1.879	& \textbf{1.875} 	& 16 	& 16\\
\cline{2-12}
& $0.1$ &  0.161	& 0.3684	& \textbf{0.1555}	& 0.1565 	&  1.484	& 1.739	& \textbf{1.469}	& 1.487 	& 15 	& 15 \\
\cline{2-12}

& $1.0$ &  0.00971	& 0.02396	& 0.00899	& \textbf{0.00876} 	&  0.4393	& 0.6923	& 0.4256	& \textbf{0.418} 	& 11 	& 9 \\
\cline{2-12}
& $1.5$ &  0.00473	& 0.00822	& 0.004	& \textbf{0.00384} 	&  0.3074	& 0.4042	& 0.2838	& \textbf{0.2779} 	& 9 	& 6 \\
\cline{2-12}
&$2.0$ 	&  0.00261	& 0.00308	& 0.00211	& \textbf{0.00188} 	&  0.2285	& 0.2476	& 0.2059	& \textbf{0.1954} 	& 7 	& 4 \\
\cline{2-12}
&$3.0$ 	&  0.0011	& 0.00056	& 0.00074	& \textbf{0.00055} 	&  0.1495	& 0.1053	& 0.1221	& \textbf{0.1051} 	& 4 	& 2 \\
\cline{1-12}

\multicolumn{1}{|c|}{\multirow{7}{*}{64}} & $0.1$ &  0.1543	& 0.4348	& 0.1536	& \textbf{0.1519} 	&  1.691	& 1.88	& \textbf{1.69}	& \textbf{1.69} 	& 31 	& 30 \\
\cline{2-12}
& $0.5$ &  0.03388	& 0.105	& \textbf{0.03359}	& 0.03383 	&  1.114	& 1.578	& \textbf{1.107}	& 1.11 	& 27 	& 24 \\
\cline{2-12}
& $1.0$ &  0.01476	& 0.04257	& 0.01414	& \textbf{0.01383} 	&  0.7649	& 1.213	& 0.7439	& \textbf{0.7397} 	& 22 	& 17 \\
\cline{2-12}
& $1.5$ &  0.00789	& 0.0193	& 0.0072	& \textbf{0.0068} 	&  0.5603	& 0.8649	& 0.5343	& \textbf{0.5209} 	& 17 	& 12 \\
\cline{2-12}
&$2.0$ 	&  0.00476	& 0.00882	& 0.00403	& \textbf{0.00368} 	&  0.4358	& 0.5903	& 0.3998	& \textbf{0.3823} 	& 13 	& 8 \\
\cline{2-12}
&$3.0$ 	&  0.00206	& 0.00162	& 0.00141	& \textbf{0.00113} 	&  0.2872	& 0.2538	& 0.2382	& \textbf{0.212} 	& 7 	& 3 \\
\cline{2-12}
&$5.0$ 	&  0.00058	& 9.97e-05	& 0.000189	& \textbf{9.95e-05} 	&  0.1523	& 0.06337	& 0.0873	& \textbf{0.06334} 	& 2 	& 1 \\
\cline{1-12}

\multicolumn{1}{|c|}{\multirow{5}{*}{$2^7$}} & $0.1$ &  0.148	& 0.523	& \textbf{0.1431}	& 0.1456 	&  1.824	& 1.95	& \textbf{1.823}	& 1.824 	& 62 	& 61 \\
\cline{2-12}
& $1.0$ &  0.01723	& 0.05896	& 0.01675	& \textbf{0.01658} 	&  1.122	& 1.61	& 1.108	& \textbf{1.103} 	& 43 	& 34 \\
\cline{2-12}
&$2.0$ 	&  0.00715	& 0.01694	& 0.00634	& \textbf{0.00591} 	&  0.7504	& 1.107	& 0.7083	& \textbf{0.6832} 	& 26 	& 15 \\
\cline{2-12}
&$3.0$ 	&  0.00358	& 0.00436	& 0.00263	& \textbf{0.00222} 	&  0.5339	& 0.5858	& 0.4573	& \textbf{0.4203} 	& 14 	& 6 \\
\cline{2-12}
&$5.0$ 	&  0.0011	& 0.00025	& 0.00047	& \textbf{0.00024} 	&  0.2964	& \textbf{0.1379}	& 0.1934	& 0.1385 	& 4 	& 1 \\
\cline{1-12}

\multicolumn{1}{|c|}{\multirow{4}{*}{$2^8$}} & $1.0$ &   0.01753	& 0.07743	& 0.01726	& \textbf{0.01703} 	&  1.432	& 1.83	& 1.424	& \textbf{1.417} 	& 87 	& 69 \\
\cline{2-12}
&$2.0$ 	&  0.00846	& 0.02386	& 0.0078	& \textbf{0.00735} 	&  1.112	& 1.539	& 1.077	& \textbf{1.049} 	& 53 	& 31 \\
\cline{2-12}
&$3.0$ 	&  0.0049	& 0.00826	& 0.004	& \textbf{0.00345} 	&  0.8757	& 1.093	& 0.7928	& \textbf{0.7389} 	& 29 	& 12 \\
\cline{2-12}
&$5.0$ 	&  0.00187	& 0.000599	& 0.000863	& \textbf{0.00055} 	&  0.5447	& 0.3074	& 0.3707	& \textbf{0.2944} 	& 7 	& 2 \\
\hline
\end{tabular}
\end{table}
\vspace*{-2em}

proof of which is presented at Appendix \ref{app:l2k}.


In these experiments, $n=10000$ data providers (participants) are simulated, the privacy level $\epsilon$ ranges from $0.01$ to $5.0$ and the data domain size $d$ ranges from $2$ to $256$. During each simulation, the truly distribution $\theta$ is generated randomly, the estimated distribution $\hat{\theta}$ is postprocessed and optimized by projecting onto probability simplex \citep{wang2013projection}\citep{duchi2008efficient}. Numerical results are mean error of $100$ repeated simulations.

Under the measurement of $\|\hat{\theta}-\theta\|_2^2$ or $\|\hat{\theta}-\theta\|_1$, the $l_2$-norm optimal mechanism $k^\#$-SS achieves slightly better performance than the mutual information optimal mechanism $k^*$-SS, but the difference is pretty minor.


We notice that there are some other local private mechanisms by adding noises (e.g. Laplace noises \citep{dwork2006calibrating}, two-sided geometric noises \citep{ghosh2009universally}\citep{geng2015staircase}) on secret data that represented as bit maps, but their mutual information bounds or distribution estimation performances are dominated by their binary version: binary randomized response.


